Learning to Optimize Multigrid PDE Solvers

Constructing fast numerical solvers for partial differential equations (PDEs) is crucial for many scientific disciplines. A leading technique for solving large-scale PDEs is using multigrid methods. At the core of a multigrid solver is the prolongation matrix, which relates between different scales of the problem. This matrix is strongly problem-dependent, and its optimal construction is critical to the efficiency of the solver. In practice, however, devising multigrid algorithms for new problems often poses formidable challenges. In this paper we propose a framework for learning multigrid solvers. Our method learns a (single) mapping from a family of parameterized PDEs to prolongation operators. We train a neural network once for the entire class of PDEs, using an efficient and unsupervised loss function. Experiments on a broad class of 2D diffusion problems demonstrate improved convergence rates compared to the widely used Black-Box multigrid scheme, suggesting that our method successfully learned rules for constructing prolongation matrices.

==> evaluation.tex <==
Several evaluation methods are in order. 
The network is trained to minimized the Frobenious norm of the iteration matrix of rather small grids made of circulant blocks and periodic boundary conditions. 
To see if the network can function as a PDE solver, and what boost it brings about compared to the standard benchmark, we report the following evaluations.
\begin{enumerate}
    \item \textit{Spectral radius} of iterations matrices of problems with large grid sizes, where no block-circulancy is assumed, and with Dirichlet boundary conditions (which are more common in practice).
    \item In practice, a two-level scheme is too expensive as the coarse grid system remains too large to be solved directly. 
    Therefore, the coarse grid system is also solved using a multi grid approach recursively. When the coarse grid system is approximated with one cycle of a multi grid scheme, it is called a \textit{v-cycle}, and when two cycles are done at each coarse level, it is called a \textit{w-cycle}. 
    It is therefore necessary to evaluate the network on a full v-cycle and w-cycle, where the same network is used in all recursion levels.
    \item The diffusion problems given to the network during training were with     $\varepsilon=0$, however, the network is evaluated on $\varepsilon \in [0,1]$ as well.
    \item Another evluation we employ is test generalization to other distributions, such as a uniform distribution over $g$ instead of the log-normal that was used for training.
\end{enumerate}


